Proteins with greater influence on network dynamics evolve more slowly but are not more essential

A fundamental question for evolutionary biology is why rates of evolution vary dramatically between proteins. Perhaps surprisingly, it is controversial how much a protein's functional importance affects its rate of evolution. In most studies, functional importance has been measured on the coarse scale of protein knock-outs, while evolutionary rate has been measured on the fine scale of amino acid substitutions. Here we introduce dynamical influence, a finer measure of protein functional importance. To measure dynamical influence, we first use detailed biochemical models of particular reaction networks to measure the influence of each reaction rate constant on network dynamics. We then define the dynamical influence of a protein to be the average influence of the rate constants for all reactions it is involved in. Using models of a dozen biochemical systems and sequence data from vertebrates, we show that dynamical influence and evolutionary rate are negatively correlated; proteins with greater dynamical influence evolve more slowly. We also show that proteins with greater dynamical influence are not more likely to be essential. This suggests that there are many cellular reactions whose presence is essential for life, but whose quantitative rate is relatively unimportant to fitness. We also provide evidence that the effect of dynamical influence on evolutionary rate is independent of protein expression level, expression specificity, gene compactness, and reaction degree. Dynamical influence offers a finer view of functional importance, and our results suggest that focusing on essentiality may have previously led to an underestimation of the role function plays in protein evolution.

==> Nrxn.tex <==
\begin{tabular}{cccc}
system & $r_{dN/dS,Nrxn}$ (p-val, N) & $r_{D,Nrxn}$ (p-val, N) & $r_{dN/dS,D|Nrxn}$\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & +0.12 (0.65, 13) & +0.32 (0.86, 13) & -0.42\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & +0.03 (0.55, 14) & -0.60 (0.01, 14) & -0.31\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & -0.16 (0.35, 8) & -0.40 (0.17, 8) & -0.79\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & +0.05 (0.57, 17) & +0.23 (0.82, 17) & -0.45\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.40 (0.02, 25) & -0.27 (0.09, 25) & -0.24\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & -0.43 (0.11, 10) & -0.47 (0.09, 10) & -0.66\\
IL6 signaling \cite{bib:Singh2006} & -0.42 (0.03, 10) & +0.37 (0.82, 10) & -0.14\\
G1 cell cycle progression \cite{bib:Haberichter2007} & -0.32 (0.20, 10) & -0.32 (0.18, 10) & -0.45\\
Rho-kinase activation \cite{bib:Maeda2006} & -0.02 (0.52, 16) & -0.26 (0.10, 16) & -0.22\\
Arachidonic acid metabolism \cite{bib:Yang2007} & +0.03 (0.53, 10) & -0.26 (0.25, 10) & -0.54\\
TNF-driven apoptosis \cite{bib:Albeck2008} & --- & --- & ---\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & +0.15 (0.68, 10) & -0.54 (0.05, 10) & +0.57\\
\hline
expected sign & $-$ & $+$ & $-$ \\
 total of expected sign & 6 & 3 & 10 \\
\end{tabular}

==> SupplementaryData/README <==
Each directory corresponds to a model. 

hessian.dat is the full \Chi^2-hessian. hessian_keys.dat lists the parameters in the order they enter the hessian. For this paper, we're only using the diagonal components.

The .py files in the directories are:
Nets.py: Creates the Networks (conditions) that we'll consider for the model.
reproduction.py: When run, produces graphs for the various conditions that can
                 be compared with the original publication to help confirm that
                 we've successfully implemented their model.

To generate the \Chi^2-Hessians for a specific model, use
python runModels.py <model directory name>

When finished, the model directory will contain a number of hess_dict.*.bp files, one for each condition. These correspond to the individual terms in the sum for H^{\chi^2}. It will also regenerate hessian.dat and hessian_keys.dat.

Each directory also contains a data.csv file that records all the data collected about a protein. These include the identifiers used for other databases, species used in alignment, etc.


==> compactness.tex <==
\begin{tabular}{cccc}
system & $r_{dN/dS,C}$ (p-val, N) & $r_{D,C}$ (p-val, N) & $r_{dN/dS,D|C}$\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & +0.11 (0.62, 11) & +0.50 (0.94, 11) & -0.49\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & +0.20 (0.75, 14) & +0.01 (0.53, 14) & -0.27\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & +0.29 (0.74, 7) & -0.39 (0.20, 7) & -0.59\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & +0.00 (0.52, 16) & -0.11 (0.38, 16) & -0.41\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.01 (0.50, 25) & +0.39 (0.96, 25) & -0.11\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & +0.73 (0.99, 10) & -0.31 (0.19, 10) & -0.15\\
IL6 signaling \cite{bib:Singh2006} & +0.07 (0.69, 10) & +0.63 (0.96, 10) & -0.41\\
G1 cell cycle progression \cite{bib:Haberichter2007} & +0.41 (0.88, 10) & +0.25 (0.76, 10) & -0.46\\
Rho-kinase activation \cite{bib:Maeda2006} & +0.74 (1.00, 16) & -0.34 (0.06, 16) & +0.07\\
Arachidonic acid metabolism \cite{bib:Yang2007} & -0.55 (0.06, 10) & +0.28 (0.81, 10) & -0.47\\
TNF-driven apoptosis \cite{bib:Albeck2008} & -0.44 (0.07, 12) & +0.04 (0.58, 12) & -0.14\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & +0.22 (0.75, 10) & -0.41 (0.14, 10) & +0.54\\
\hline
expected sign & $+$ & $-$ & $-$ \\
 total of expected sign & 9 & 5 & 10 \\
\end{tabular}

==> supp_dN_dS.tex <==
\begin{tabular}{ccc}
system & $r_{dN,D}$ (p-val, N) & $r_{dS,D}$ (p-val, N)\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & -0.29 (0.17, 13) & -0.40 (0.09, 13)\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & -0.25 (0.20, 14) & -0.30 (0.15, 14)\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & -0.65 (0.03, 8) & -0.46 (0.11, 8)\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & -0.41 (0.03, 17) & -0.01 (0.46, 17)\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.07 (0.39, 25) & -0.16 (0.22, 25)\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & -0.34 (0.16, 10) & +0.29 (0.79, 10)\\
IL6 signaling \cite{bib:Singh2006} & -0.04 (0.50, 9) & +0.04 (0.55, 9)\\
G1 cell cycle progression \cite{bib:Haberichter2007} & -0.41 (0.13, 9) & -0.22 (0.30, 9)\\
Rho-kinase activation \cite{bib:Maeda2006} & -0.32 (0.09, 15) & +0.36 (0.93, 15)\\
Arachidonic acid metabolism \cite{bib:Yang2007} & -0.17 (0.32, 10) & +0.56 (0.92, 10)\\
TNF-driven apoptosis \cite{bib:Albeck2008} & +0.21 (0.74, 11) & -0.33 (0.15, 11)\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & +0.35 (0.80, 8) & +0.07 (0.56, 8)\\
\hline
expected sign & $-$ & $-$ \\
 total of expected sign & 10 & 7 \\
\end{tabular}

==> supp_important.tex <==
\begin{tabular}{ccc}
system & $r_{dN/dS,D}$ (p-val, N) & ``output'' variables\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & -0.24 (0.23, 12) & active ERK\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & -0.33 (0.16, 12) & active ERK and active Akt\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & -0.73 (0.03, 8) & active ERK\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & -0.40 (0.05, 16) & active ERK\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.19 (0.21, 24) & active ERK\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & -0.02 (0.54, 10) & $\beta$-catenin/TCF complex\\
IL6 signaling \cite{bib:Singh2006} & -0.05 (0.69, 9) & nuclear STAT3\\
G1 cell cycle progression \cite{bib:Haberichter2007} & -0.57 (0.05, 9) & hypo- and hyper-phosphorylated Rb\\
Rho-kinase activation \cite{bib:Maeda2006} & -0.19 (0.28, 15) & phosphorylated myosin light chain\\
Arachidonic acid metabolism \cite{bib:Yang2007} & -0.57 (0.05, 10) & PGE2 and LTB4\\
TNF-driven apoptosis \cite{bib:Albeck2008} & -0.22 (0.34, 12) & the apoptosome\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & -0.18 (0.32, 9) & active MAP kinase\\
\hline
expected sign & $-$ \\
 total of expected sign & 12 \\
\end{tabular}

==> supp_mammals.tex <==
\begin{tabular}{cc}
system & $r_{dN/dS,D}$ (p-val, N)\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & -0.28 (0.17, 13)\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & -0.23 (0.21, 14)\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & -0.58 (0.07, 8)\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & -0.27 (0.15, 17)\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.03 (0.45, 25)\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & -0.37 (0.14, 10)\\
IL6 signaling \cite{bib:Singh2006} & -0.30 (0.21, 10)\\
G1 cell cycle progression \cite{bib:Haberichter2007} & -0.31 (0.19, 10)\\
Rho-kinase activation \cite{bib:Maeda2006} & -0.10 (0.40, 16)\\
Arachidonic acid metabolism \cite{bib:Yang2007} & -0.49 (0.08, 10)\\
TNF-driven apoptosis \cite{bib:Albeck2008} & -0.11 (0.41, 12)\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & +0.70 (0.98, 9)\\
\hline
expected sign & $-$ \\
 total of expected sign & 11 \\
\end{tabular}

==> supp_unique.tex <==
\begin{tabular}{cc}
system & $r_{dN/dS,D}$ (p-val, N)\\
\hline
Insulin/EGF signaling \cite{bib:Borisov2009} & -0.61 (0.08, 6)\\
Heregulin/EGF signaling \cite{bib:Birtwistle2007} & -0.63 (0.06, 6)\\
NGF/EGF signaling (smaller) \cite{bib:Brown2004} & --- (---, 1)\\
NGF/EGF signaling (larger) \cite{bib:Sasagawa2005} & -0.39 (0.21, 7)\\
EGF receptor endocytosis \cite{bib:Ung2008} & -0.01 (0.49, 10)\\
Wnt/ERK crosstalk \cite{bib:Kim2007} & -0.42 (0.16, 7)\\
IL6 signaling \cite{bib:Singh2006} & -0.28 (0.24, 10)\\
G1 cell cycle progression \cite{bib:Haberichter2007} & -0.31 (0.19, 10)\\
Rho-kinase activation \cite{bib:Maeda2006} & -0.26 (0.20, 14)\\
Arachidonic acid metabolism \cite{bib:Yang2007} & -0.53 (0.06, 10)\\
TNF-driven apoptosis \cite{bib:Albeck2008} & -0.14 (0.36, 12)\\
$\beta$-adrenergic signaling \cite{bib:Neves2008} & +0.26 (0.71, 7)\\
\hline
expected sign & $-$ \\
 total of expected sign & 10 \\
\end{tabular}
